Estimating Uncertainty of Omnimodal Large Language Models via External Omnimodal Embeddings

Recent work has investigated Omni-modal Large Language Models (OLLMs), models which can take multiple modalities and their combinations as input, as a way forward to have systems really capable of interacting with their environment. Uncertainty quantification (UQ) for OLLMs, however, remains an open problem: existing methods largely target at most two modalities at a time, require access to model internals, or re-invocation of the evaluated model. We propose a model-agnostic UQ framework that scores a Chain-of-Thought response entirely through external omni-modal embeddings, measuring the grounding of the reasoning in the multimodal input and its internal coherence. Our contribution is the family of signals and an empirical characterisation of when it is reliable, rather than any single estimator: we find the geometric scores to be largely redundant with one another (mean within-split rank correlation 0.91-0.94) but strongly complementary to answer-dispersion baselines, and their reliability to depend on the generator and the modality. The resulting confidence estimates require no access to logits, hidden states or gradients of the evaluated model and no additional inference from it; they do require segmenting the reasoning trace with an auxiliary model and, for the aggregated score, a labelled calibration set that we show can be as small as 25 examples (although we also show that such a set buys little over fixing one signal a priori). On UNO-Bench, with both a closed and an open model, our scores yield small gains over self-consistency (systematic with the closed generator, mixed with the open one) and are competitive with self-verbalisation and internal-state baselines, especially in open-ended, omni-modal questions where previous state-of-the-art baselines struggle.

==> sections/appendices/artifact_description.tex <==
\section{Artifact Documentation.}
Our experiments use UNO-Bench, a unified benchmark for evaluating omni-modal large language models across both uni-modal and omni-modal understanding capabilities. UNO-Bench comprises 44 task types spanning perception and reasoning abilities under a unified capability taxonomy, covering image, video, audio, and text modalities as well as their combinations. The benchmark contains 1,250 human-curated omni-modal samples and 2,480 enhanced uni-modal samples, with the omni-modal portion designed such that approximately 98\% of the questions require information from multiple modalities for successful resolution.

UNO-Bench includes both multiple-choice and multi-step open-ended questions, enabling the evaluation of perception, cross-modal alignment, temporal reasoning, spatial reasoning, and complex multi-step reasoning. The benchmark covers diverse application domains, including everyday scenarios, society, culture, art, science, mathematics, document understanding, and audiovisual reasoning, using real-world images, videos, and human-recorded audio.

The benchmark contains both English and Chinese data. In particular, the manually curated omni-modal dataset was designed to better reflect real-world scenarios in Chinese linguistic contexts while also including English-language content. Human annotators, including domain experts and crowd workers, constructed the benchmark through a human-centric annotation pipeline with multiple rounds of model-assisted and manual quality control.

UNO-Bench was not specifically designed for fairness or demographic evaluation. Although the collected multimedia content includes people from a variety of real-world contexts, the benchmark does not provide demographic annotations or guarantee balanced representation across demographic groups. Consequently, our evaluation does not support conclusions regarding fairness or subgroup performance.

As UNO-Bench is a benchmark for evaluating multimodal understanding rather than demographic characteristics, any biases present in the underlying media, annotations, or cultural contexts may be reflected in model performance. We therefore interpret our uncertainty estimation results as measurements of model calibration on the benchmark tasks rather than indicators of fairness or general societal performance.


==> sections/appendices/sampling_free.tex <==
\section{The Strictly Single-Generation Regime}
\label{app:single-chain}
\label{sec:single-chain}

The main protocol scores a fixed, majority-selected answer and, for the embedding-based methods, forms the confidence by aggregating per-chain scores over the candidate pool (the sum-share of Section~\ref{sec:experimental-setup}). The cheapest conceivable deployment instead produces \emph{exactly one} chain and scores it in isolation; this appendix evaluates that regime directly. Each question is represented by its first sampled generation (all candidates are exchangeable draws at temperature 1.0), scored by its own per-chain value, with that generation's own correctness as the label; no clustering or aggregation of any kind is used. $\mathcal{C}_{\text{chain}}$ is refitted on the canonical partition's validation items under the published protocol, with model selection likewise performed single-chain. Table~\ref{tab:single-chain} reports the results (ECE is omitted: in this regime it is governed by the same scale artefacts analysed in Appendix~\ref{app:variance}, and Platt calibration applies unchanged).

\begin{table*}[t]
\centering
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{l cc cc cc cc cc}
\toprule
& \multicolumn{2}{c}{Avg} & \multicolumn{2}{c}{Audio} & \multicolumn{2}{c}{MC} & \multicolumn{2}{c}{MO} & \multicolumn{2}{c}{Visual} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
Method & AUROC & AURAC & AUROC & AURAC & AUROC & AURAC & AUROC & AURAC & AUROC & AURAC \\
\midrule
Level-Based Conf. & 0.557 & 0.670 & 0.540 & 0.843 & 0.531 & 0.602 & 0.583 & 0.411 & 0.573 & 0.823 \\
Self-Probing Conf. & \textbf{0.629} & \textbf{0.715} & 0.610 & 0.857 & \textbf{0.590} & \textbf{0.666} & \textbf{0.671} & 0.483 & \textbf{0.643} & \textbf{0.852} \\
Two-Step CoT Conf. & 0.608 & 0.707 & 0.600 & 0.862 & 0.568 & 0.624 & 0.663 & \textbf{0.499} & 0.602 & 0.841 \\
\midrule
$S_{\text{smooth}}$ & 0.476 & 0.629 & 0.521 & 0.823 & 0.497 & 0.596 & 0.392 & 0.348 & 0.494 & 0.750 \\
$S_{\text{dens}}$ & 0.471 & 0.621 & 0.493 & 0.802 & 0.494 & 0.593 & 0.422 & 0.341 & 0.476 & 0.747 \\
$S_{\text{goal}}$ & 0.514 & 0.648 & 0.459 & 0.802 & 0.524 & 0.612 & 0.545 & 0.400 & 0.527 & 0.778 \\
$G_{\text{avg}}$ & 0.498 & 0.641 & 0.482 & 0.808 & 0.520 & 0.613 & 0.477 & 0.375 & 0.512 & 0.766 \\
$G_{\max}$ & 0.547 & 0.677 & \textbf{0.614} & \textbf{0.868} & 0.525 & 0.623 & 0.537 & 0.431 & 0.512 & 0.786 \\
\midrule
$\mathcal{C}_{\text{chain}}$ & 0.527 & 0.671 & 0.509 & 0.833 & 0.506 & 0.594 & 0.540 & 0.464 & 0.552 & 0.791 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{The strictly single-generation regime: AUROC and AURAC ($\uparrow$) when exactly one chain per question is scored by its own value (Gemini-generated answers, canonical test partition; no clustering or pool aggregation). Sampling-based methods do not exist in this regime. Avg is the unweighted mean of the four per-split values; bold marks the best value per column. The corresponding pooled-union values are reported in Appendix~\ref{app:overall}, where the $\mathcal{C}_{\text{chain}}$ row of this regime serves as the starkest example of the pooling bias: its pooled AUROC of 0.653 against near-chance per-split values.}
\label{tab:single-chain}
\end{table*}

Three findings follow. First, the coherence scores and $G_{\text{avg}}$ \emph{collapse to chance} (0.47--0.51 average AUROC): their discriminative power in the main protocol comes from the sum-share aggregation over the candidate pool, whose value is dominated by cluster size, i.e.\ by the agreement signal of the samples. They are therefore ensemble-level evidence, not properties of an individual chain that predict its correctness — which is consistent with, and motivates, their use as vote weights in Appendix~\ref{app:gwsc}. Second, $G_{\max}$ is the exception: it retains genuine single-chain signal (0.614 AUROC on Audio, where the candidate-pool protocol fails at 0.435) and attains the best average AUROC (0.547) and AURAC (0.677) among the geometric scores, so maximal step-to-input grounding is the one geometric quantity in our set that is informative about a chain in isolation. Third, the self-verbalisation baselines, which are single-chain by construction, dominate discrimination in this regime (Self-Probing 0.629 average AUROC and 0.715 average AURAC), at the cost of one additional call to the evaluated model. A related experiment in which each method \emph{selects} the answer purely by its own per-candidate score (a best-of-$n$ policy) degrades both accuracy and every UQ metric relative to majority voting for all methods, confirming the same reading: the geometric scores' value lies in modulating the ensemble, not in ranking candidates within a question.

==> sections/appendices/software_environment.tex <==
\section{Software Environment}

All experiments were implemented in Python and executed using widely adopted open-source machine learning and scientific computing libraries. Table~\ref{tab:packages} summarizes the primary software dependencies used in our implementation.

\begin{table}[ht]
\centering
\small
\begin{tabular}{ll}
\toprule
\textbf{Package} & \textbf{Version} \\
\midrule
Python & 3.12 \\
numpy & 2.3.2 \\
pandas & 2.3.1 \\
scipy & 1.16.1 \\
scikit-learn & 1.7.1 \\
torch & 2.8.0 \\
torchvision & 0.23.0 \\
transformers & 4.56.0 \\
huggingface-hub & 0.34.4 \\
sentence-transformers & 5.1.0 \\
accelerate & 1.10.0 \\
tokenizers & 0.22.0 \\
safetensors & 0.6.2 \\
google-genai & 1.30.0 \\
tqdm & 4.67.1 \\
Pillow & 11.3.0 \\
opencv-python & 4.12.0 \\
matplotlib & 3.10.5 \\
seaborn & 0.13.2 \\
PyYAML & 6.0.2 \\
\bottomrule
\end{tabular}
\caption{Primary software dependencies used in our implementation.}
\label{tab:packages}
\end{table}

All pretrained models and datasets were obtained through their official releases via the Hugging Face ecosystem or the corresponding model providers. Experiments were conducted using deterministic random seeds whenever applicable. The complete source code, configuration files, and dependency specifications will be released to facilitate reproducibility.


==> sections/figure_method.tex <==
% Methodology overview figure (TikZ). All formulas transcribed verbatim from
% sections/methodology.tex — keep the two in sync if the equations change.
\resizebox{\textwidth}{!}{%
\begin{tikzpicture}[
    >=Stealth,
    node distance=0.55cm and 0.55cm,
    box/.style={draw, rounded corners, align=center, font=\scriptsize, inner sep=5pt},
    panel/.style={draw, thick, rounded corners, align=left, font=\scriptsize, inner sep=6pt},
]
% ---- top row: pipeline ----
\node[box, fill=blue!5, text width=3.4cm] (inputs) {%
    \textbf{Inputs}\\[2pt]
    multimodal context\\
    $\mathcal{V}=\{V^{(1)},\dots,V^{(K)}\}$\\
    (image\,/\,audio\,/\,text\,/\,\dots)\\[3pt]
    \textbf{Black-box OLLM} $\mathcal{M}$\\
    (e.g., Gemini, MiniCPM-o)};
\node[box, fill=gray!10, right=of inputs, text width=2.7cm] (chain) {%
    \textbf{Reasoning chain}\\[2pt]
    $R=(r_1,\dots,r_m)$\\[2pt]
    final answer $a$};
\node[box, fill=blue!15, right=of chain, text width=3.1cm] (enc) {%
    \textbf{External omnimodal}\\
    \textbf{embedding model} $\mathcal{E}$\\[2pt]
    (e.g., E5-Omni,\\ LCO-Embedding-Omni)};
\node[box, fill=blue!5, right=of enc, text width=3.5cm] (emb) {%
    \textbf{Shared embedding space}\\[2pt]
    inputs: $\Phi^{(k)}=\mathcal{E}(V^{(k)})$\\
    steps: $\phi_{r_1},\dots,\phi_{r_m}$\\
    answer: $\phi_a$};
\draw[->] (inputs) -- (chain);
\draw[->] (chain) -- (enc);
\draw[->] (enc) -- (emb);
\draw[->] (inputs.south) to[bend right=15]
    node[below, font=\tiny, yshift=-2pt]{inputs are embedded directly} (enc.south);

% ---- middle row: score panels ----
\node[panel, fill=violet!8, text width=7.0cm, minimum height=3.4cm, anchor=north west]
    (ground) at ([xshift=-0.1cm, yshift=-1.5cm]inputs.south west) {%
    \textbf{A. Grounding} (alignment with the inputs)\\[5pt]
    per-modality alignment of step $r_i$:\\[2pt]
    \hspace*{6pt}$A^{(k)}(r_i)=\max_{\phi_v\in\Phi^{(k)}}\mathcal{S}(\phi_{r_i},\phi_v)$\\[4pt]
    omnimodal alignment:\\[2pt]
    \hspace*{6pt}$A^{\mathrm{omni}}(r_i)=\max_{k=1,\dots,K}A^{(k)}(r_i)$\\[4pt]
    aggregation over steps:\\[2pt]
    \hspace*{6pt}$G_{\text{avg}}=\frac{1}{m}\sum_{i=1}^{m}A^{\mathrm{omni}}(r_i)$,\quad
    $G_{\max}=\max_{i}A^{\mathrm{omni}}(r_i)$};
\node[panel, fill=green!8, text width=7.6cm, minimum height=3.4cm, anchor=north east]
    (coh) at ([xshift=0.1cm, yshift=-1.5cm]emb.south east) {%
    \textbf{B. Coherence} (internal geometry of the chain)\\[5pt]
    local smoothness:\;
    $S_{\text{smooth}}=\frac{1}{m-1}\sum_{i=1}^{m-1}\mathcal{S}(\phi_{r_i},\phi_{r_{i+1}})$\\[4pt]
    semantic density:\;
    $S_{\text{dens}}=\frac{1}{m(m-1)}\sum_{i\neq j}\mathcal{S}(\phi_{r_i},\phi_{r_j})$\\[4pt]
    answer convergence:\;
    $S_{\text{goal}}=\gamma\,\mu_{\text{goal}}+(1-\gamma)\,\Delta_{\text{goal}}$,\; $\gamma=0.6$\\[2pt]
    \hspace*{6pt}$\mu_{\text{goal}}=\frac{1}{m}\sum_{i=1}^{m}\mathcal{S}(\phi_{r_i},\phi_a)$,\;
    $\Delta_{\text{goal}}=\tfrac{1}{2}\!\left(\Delta_{\text{fwd}}-\Delta_{\text{bwd}}+1\right)$};
\draw[->] (emb.south) to[bend left=12] (coh.north);
\draw[->] ([xshift=-0.4cm]enc.south west) to[bend right=12] (ground.north);

% ---- bottom row: confidence ----
\node[panel, fill=orange!12, text width=11.2cm, align=center, anchor=north]
    (conf) at ([yshift=-0.75cm]coh.south -| chain.east) {%
    \textbf{Confidence estimate} (higher = less likely hallucinated)\\[3pt]
    label-free: any individual score \quad or \quad supervised aggregate:
    $\mathcal{C}_{\text{chain}}=\sigma\!\left(\mathbf{w}^{\top}\mathbf{x}+b\right)$,\;
    $\mathbf{x}=\left[S_{\text{smooth}},\,S_{\text{dens}},\,S_{\text{goal}},\,G_{\text{avg}},\,G_{\max}\right]$\\[2pt]
    (logistic regression fitted on labelled validation data)};
\draw[->] (ground.south) to[bend right=12] (conf.west);
\draw[->] (coh.south) to[bend left=12] (conf.east);
\end{tikzpicture}%
}


==> sections/limitations.tex <==
\section*{Limitations}

Our study has several limitations that qualify the scope of its conclusions.

\paragraph{Discrimination margins.} The advantage of geometry-weighted voting over plain self-consistency, while highly systematic across runs, is modest in absolute terms (just under one point of split-averaged AUROC with Gemini-generated answers and about 0.2 points with MiniCPM), most of the weighted scheme's performance is inherited from the strength of self-consistency itself, and with MiniCPM-generated answers the aggregated $\mathcal{C}_{\text{chain}}$ is essentially tied with Self-Probing and native UMPIRE on split-averaged AUROC (0.656--0.657), with both baselines holding a significant advantage under the pooled protocol of Appendix~\ref{app:overall}. Our item-level significance markers quantify generalisation to new questions from the same pool; generalisation to other benchmarks remains untested. 
%The omni-modal open-answer advantage in particular rests on a 250-question split (200 test items after the validation cut), whose item-level 95\% confidence intervals span roughly $\pm 0.08$ AUROC (Appendix~\ref{app:variance}), so we regard it as a consistent pattern across generators rather than a precisely estimated margin.

\paragraph{Calibration.} The self-verbalisation baselines are better calibrated than our scores under the range-normalised ECE protocol of Section~\ref{sec:experimental-setup}, and that protocol itself measures calibration after a split-level rescaling rather than the raw calibration a practitioner would observe at deployment. The deployment-realistic analysis of Appendix~\ref{app:variance}, with Platt scaling fitted on validation data only, shows that post-hoc calibration collapses ECE for every method and that most of the large raw-ECE gaps in the main tables are scale artefacts; the verbalised baselines retain a smaller, genuine calibrated advantage with Gemini-generated answers.

\paragraph{Supervised aggregation.} $\mathcal{C}_{\text{chain}}$ requires a modest amount of labelled validation data per split to fit the logistic-regression aggregator, whereas self-consistency and the verbalised baselines are label-free. The individual scores ($S_{\text{smooth}}$, $S_{\text{dens}}$, $S_{\text{goal}}$, $G_{\text{avg}}$, $G_{\max}$) require no training and are reported throughout as label-free alternatives. Appendix~\ref{app:transferability} tests the transferability of the learned aggregation weights across splits and generators: transfer is nearly free on average, largely because the fitted aggregator typically reduces to a validation-selected single feature, but it fails precisely where that per-split feature choice was the learned content (e.g., MiniCPM-fitted weights lose $0.046$ AUROC on Gemini-Audio).

%\paragraph{Sampling budget.} Like self-consistency, the method presupposes $N$ sampled generations per question, and its cost is self-consistency's plus one external embedding pass; we make no sampling-free claim. The coherence signals in particular behave as ensemble-level evidence over the sampled candidates, which is why we deploy them as vote weights rather than as scores for chains in isolation.

\paragraph{Audio failure mode.} All our chain-based signals, together with Self-Consistency, achieve near- or below-chance AUROC on the Audio split with Gemini-generated answers. Two observations locate this failure with the generator's answer distribution on audio questions rather than with the encoder. First, Self-Consistency is encoder-independent yet also falls below chance on this split, and Platt calibrators fitted on validation items yield \emph{negative} slopes for it and for most chain-level scores (Appendix~\ref{app:variance}): with Gemini on audio, higher agreement and higher geometric scores are anti-correlated with correctness. Second, the same chain-level features are strongly discriminative on Audio with MiniCPM-generated answers (all validation-fitted slopes strongly positive), and the dispersion of \emph{answer} embeddings from the same encoder is informative even for Gemini answers (Appendix~\ref{app:additional-baselines}), so neither the encoder's audio representations nor the chain-level signals as such are at fault. More generally, a near-chance confidence signal used to gate or escalate model outputs could give practitioners false assurance; the signal should be validated on the target modality before deployment.

\paragraph{Feature instability across generators.} The discriminative power of individual scores depends on the answer-generating model and the split: $S_{\text{goal}}$ is the second-best signal on Gemini-Visual (0.7356) yet the weakest on MiniCPM-MO (0.6462), while $G_{\max}$ is the weakest signal on Gemini-Audio (0.4351) and the strongest on MiniCPM-MO (0.6978). Per-split feature selection therefore cannot be assumed to transfer across models, and Appendix~\ref{app:aggregator-evidence} shows that the selection itself is the dominant source of error when the validation split is small.

%\paragraph{Encoder and benchmark coverage.} Our main results rely on a single external encoder (E5-Omni 3B) and a single benchmark (UNO-Bench) covering audio and vision; Appendix~\ref{app:lco-encoder} adds a second encoder, but settings with video or more than two extra-textual modalities remain untested. Moreover, as noted in Section~3, with a single shared encoder the per-modality grounding formulation reduces to its counterpart on the pooled inputs, and the systematic design of modality-aware aggregators remains open.

%\paragraph{Privacy.} Computing external embeddings requires sending potentially sensitive audio and visual inputs to a separate embedding model, which may not be acceptable in all deployment scenarios.


